Combinatorial Optimization Algorithms via Polymorphisms

An elegant characterization of the complexity of constraint satisfaction problems has emerged in the form of the the algebraic dichotomy conjecture of [BKJ00]. Roughly speaking, the characterization asserts that a CSP {\Lambda} is tractable if and only if there exist certain non-trivial operations known as polymorphisms to combine solutions to {\Lambda} to create new ones. In an entirely separate line of work, the unique games conjecture yields a characterization of approximability of Max-CSPs. Surprisingly, this characterization for Max-CSPs can also be reformulated in the language of polymorphisms. In this work, we study whether existence of non-trivial polymorphisms implies tractability beyond the realm of constraint satisfaction problems, namely in the value-oracle model. Specifically, given a function f in the value-oracle model along with an appropriate operation that never increases the value of f , we design algorithms to minimize f . In particular, we design a randomized algorithm to minimize a function f that admits a fractional polymorphism which is measure preserving and has a transitive symmetry. We also reinterpret known results on MaxCSPs and thereby reformulate the unique games conjecture as a characterization of approximability of max-CSPs in terms of their approximate polymorphisms.

==> content/conclusion.tex <==
\section{Conclusion}




==> content/descent.tex <==
\section{Black-box minimization algorithm}



The following result is a restatement of Theorem $5$ in the work of
Nesterov \cite{Nesterov11}. 


%\newcommand{\diam}{\Delta}
\begin{theorem}
	Let $\hat{f}: \R^N \to \R$ be a non-smooth convex function given by an
evaluation oracle $\cO$.  Let us suppose $f$ is
$L$-Lipshitz,i.e.,
$$ |\hat{f}(x) - \hat{f}(y)| \leq L \norm{x-y} \qquad \forall x,y \in \R^N
$$
%
Let $Q \sse \R^N$ be a closed convex set
given by a projection oracle $\pi_Q : \R^N \to Q$.  Let 
$\diam(Q) \defeq \sup_{x,y \in Q} \norm{x-y}$.

There is a randomized algorithm that given $\epsilon > 0$, with
constant probability finds $y \in
Q$ such that,
$$ |\hat{f}(y) - \min_{x \in Q} \hat{f}(x)| \leq \e\mcom$$
using $$\frac{ (N+4)L^2 \diam(Q)^2}{\epsilon^2}$$ calls to the oracle
$\cO$ and $\pi_Q$. 
\end{theorem}

In our setup, the domain $Q = \ssimp_q^n \in \R^{nq}$ is a very
simple closed convex set with diameter $\Delta(Q) \leq \sqrt{2n}$.
The convex extension $\hat{f}$ is $L$-Lipschitz for $L =
\norm{f}_\infty$.   




In this section, we will outline a randomized gradient descent
algorithm to prove the following.
\begin{theorem}
	Let $h: \ssimp_q^n \to \R$ be a convex function given by a
	value oracle $\cO$ that given $x \in \ssimp_q^n, \eta > 0$
	runs in time $\poly(n, 1/\eta)$ and returns an estimate $h(x) \pm \eta$.
	There is an algorithm that makes 
	$\poly(1/\epsilon,n,\norm{h}_{Lip}, \norm{h}_\infty)$ queries to $\cO$, runs
	in time $\poly(1/\epsilon,n,\norm{h}_{\infty}, \norm{h}_{Lip})$ and finds a $y
	\in \ssimp_q^n$ such that,
	$$ h(y) \leq \min_{x \in \ssimp_q^n} h(x) + \epsilon \norm{h}_\infty$$
\end{theorem}

The function $h$ need not be diffrentiable.  We begin by
constructing a smooth function $g$ that approximates $h$ well.

Let $V_q \subset \R^q$ denote the subspace,
$V_q = \{x \in \R^q| \sum_{i \in [q]} x_i = 0\}$.  Fix $V = V_q^n$.
Let $B_V(x,\eta) \sse V$ denote the $\ell_2$-ball of radius $\eta$ around $x
\in V$.

Define the convex set $\cC_{\eta}$ as follows,
$$ \cC_{\eta} = \{ x \in \ssimp_{q}^n |  B(x,\eta) \subset \ssimp_q^n
\} \mcom$$
where $B_V(x,\eta)$ is the ball of radius $\eta$ around $x$.

Let $\Psi : \R^{qn} \to \R^+$ be a thrice-differentiable function such
that, 
$$ \Psi(z) = 0 \qquad \qquad \forall z \notin B_V\left(0,\frac{\eta}{2}\right) \mcom$$
$$ \int_{z \in \R^n} \Psi(z) dz = 1 \mcom$$
and $\norm{\Psi'}_{\infty}, \norm{\Psi''}_\infty \leq
c(n,1/\eta)$ for some polynomial in $n$ and $\eta$.
Define the function $g : \cC_{\eta} \to \R$ as,
$$ g(x) \defeq \int_{z \in \R^n} h(x+z) \Psi(z) dz $$
It is easy to check that the function $g$ satisfies the following
properties:
\begin{enumerate}
\item $g$ is thrice differentiable and convex.
\item For each $x \in \cC_{\eta}$, $\| g(x) - h(x) \| \leq \eta \cdot
\norm{h}_{Lip}$.  Moreover, 
$$ \min_{x \in \cC_\eta} g(x) \leq \min_{x \in \ssimp_q^n} h(x) +
2\eta \norm{h}_{Lip} \mper$$.
\item $ \max_{x \in \cC_{\eta}} \norm{H_g(x)} \leq c(n,1/\eta)\norm{h}_\infty
\mcom$
   where $H_g(x)$ is the Hessian of $g$ evaluated at $x$.
\item For any $\delta > 0$ and $x \in \cC_{\eta}$, the value of $g(x)$
can be estimated within error $\delta$ in time
$\poly(n,1/\eta,1/\delta, \norm{h}_\infty)$ given access to oracle
$\cO$.
\end{enumerate}

\begin{theorem}
	Let $\cC$ be a convex set given by the separation oracle and
	let $g : \cC \to \R$ be a thrice-diffrentiable convex function
	on $\cC$.  Let $\cO$ be an oracle that given $x \in \cC$ and
	$\delta$, returns an approximation $t \in [g(x)-\delta,
		g(x)+\delta]$ in time $\poly(n, 1/\delta)$.  There is
		an efficient algorithm that for every $\eta$, finds a $y \in \cC$ such
		that $g(y) \leq \min_{x \in \cC} g(x) + \eta
		\norm{g}_\infty$ in
		oracle time
		$\poly(n, 1/\eta, \norm{g}_\infty, \norm{g'}_\infty,
		\norm{g''}_\infty, D)$ where $D$ is
		the diameter of the convex set $\cC$.
\end{theorem}

\begin{proof}
The oracle $\cO$ is an evaluation oracle for $g$, but does not yield
the gradient directly.  However, there are numerous approaches to
estimate the gradient of $g$ and use it to perform a gradient descent.
These have been extensively studied in stochastic
approximation/stochastic gradient descent. One possible approach is
outlined by Spall \cite{Spall97}, but there are numerous other works
(see \cite{FlaxmanKalai05} and references therein) . 

\end{proof}



==> content/oldnotex.tex <==
\paragraph{Product Distribution vs Correlated Distribution}
Let $\mu$ be a probability distribution over $[q]^n$.  Let $X_1, \ldots, X_n$ be
the jointly distributed $[q]$-valued random variables associated with
$\mu$.  For each $i \in [n]$, let $\rho_i =
\rho(X_{1,\ldots,i-1},X_i)$. Let $\mu^{\times}$ denote the probability distribution $\mu_1 \times
\mu_2 \times \ldots \times \mu_n$.
%\vspace{-10pt}
\begin{lemma}\label{lem:corrvsind}
	\begin{displaymath}\norm{\cP^{\otimes r}(\mu) - \cP^{\otimes
	r}(\mu^{\times})}_1 \leq \sum_{i \in [n]} \rho_i
\left(1 - (1-\Lin(\cP))(1-\rho_i^2)\right)^r\end{displaymath} 
\end{lemma}
%\vspace{-10pt}
\begin{proof}
	An easy consequence of \prettyref{lem:correlation-decay-poly}
	and \prettyref{lem:corr-stat-distance}.  Specifically, for
	each $i$ starting from $n$ to $1$, replace the $i^{th}$
	coordinate in $\cP^{\otimes r}(\mu)$ by an independent random
	variable with same marginal.  The statistical distance or
	error accrued in each step is at most $\rho_i
\left(1 - (1-\Lin(\cP))(1-\rho_i^2)\right)^r$ by
\prettyref{lem:correlation-decay-poly} and
\prettyref{lem:corr-stat-distance}. 
\end{proof}



